Estimation and Visualization of Isosurface Uncertainty from Linear and High-Order Interpolation Methods

Isosurface visualization is fundamental for exploring and analyzing 3D volumetric data. Marching cubes (MC) algorithms with linear interpolation are commonly used for isosurface extraction and visualization. Although linear interpolation is easy to implement, it has limitations when the underlying data is complex and high-order, which is the case for most real-world data. Linear interpolation can output vertices at the wrong location. Its inability to deal with sharp features and features smaller than grid cells can lead to an incorrect isosurface with holes and broken pieces. Despite these limitations, isosurface visualizations typically do not include insight into the spatial location and the magnitude of these errors. We utilize high-order interpolation methods with MC algorithms and interactive visualization to highlight these uncertainties. Our visualization tool helps identify the regions of high interpolation errors. It also allows users to query local areas for details and compare the differences between isosurfaces from different interpolation methods. In addition, we employ high-order methods to identify and reconstruct possible features that linear methods cannot detect. We showcase how our visualization tool helps explore and understand the extracted isosurface errors through synthetic and real-world data.

==> old/background.tex <==
\section{Technical Background}

Here, we briefly describe the MC algorithm~\cite{Willam1987} and state-of-the-art interpolation techniques used in the MC algorithm.

\subsection{MC algorithm} \label{sec:mcAlgorithm}

The MC algorithm ~\cite{Willam1987} for isosurface extraction is one of the most cited algorithms in scientific visualization literature. Given a univariate scalar function sampled on a 3D spatial domain $f: \mathbb{R}^3 \to \mathbb{R}$, isosurface represents a preimage ($S$) of a user-defined isovalue $k$, such that $S = \{\textbf{x} \in \mathbb{R}^3 | f(\textbf{x})=k\}$. 

\begin{figure}[!ht]
 \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)

 \includegraphics[width=0.98\columnwidth]{figures/MCalgorithm2D.png}
 \caption{Steps of the marching squares algorithm for a single 2D grid cell (depicted as a purple square). In step one, the isosurface topology (black contour) is determined such that it isolates vertices with $f>k$ from vertices with $f<k$. In the second step, the isocontour crossing position on a grid edge (blue cross) is estimated by linearly interpolating grid vertex values along the edge.}
 \label{fig:mcAlgo}
\end{figure}

The MC algorithm extracts the isosurface as it steps through each cell of the discrete uniform grid. Extracting the isosurface from a single grid cell comprises two steps. In the first step, the isosurface topology within the cell is determined by comparing grid vertex values with the isovalues. Specifically, isosurface topology ensures grid vertices with values greater than the isovalue and grid vertices with values smaller than the isosvalue are on two opposite sides of the isosurface. In the second step, the isosurface crossing position on grid edges is determined using the linear interpolation technique detailed in ~\autoref{sec:linear}. The two steps are depicted in the context of 2D scalar data, in \autoref{fig:mcAlgo}. Thus, the final isosurface for the entire scalar field is reconstructed through piecewise linear approximation per grid cell.

\subsection{Linear interpolation} \label{sec:linear}

Estimating isosurface orientation in the interior of each grid cell using linear approximation has advantages in terms of speed and simplicity of the mathematical model. Let $f(\textbf{x})$ and $f(\textbf{y})$ be the scalar values sampled at vertex positions \textbf{x} and \textbf{y} denoting ends of a grid edge, respectively. The crossing position for isovalue $k$ on a grid edge is determined by finding the parameter $\alpha \in [0,1]$ such that $k = \alpha*f(\textbf{y}) + (1-\alpha)*f(\textbf{x})$. The further simplification leads to $\alpha = \frac{k - f(\textbf{x})}{f(\textbf{y})-f(\textbf{x})}$.     

\subsection{Cubic interpolation}  \label{sec:cubic}

Although linear interpolation can be efficient to implement, it may lead to significant interpolation errors if the underlying function has high order. Previous efforts implemented the cubic interpolation model to enhance the accuracy of isosurface reconstruction ~\cite{Fuhrmann2015, Balazs2019, Cohen-Or2000,Marschner1994, Mitchell1988, CATMULL1974, Theisel2002}. 

For a given edge or (interval) the cubic polynomial can be expressed in terms of using monomials as follows: 
\begin{equation}\label{eq:cubiC}
q(x) = c_{0} + c_{1}x + c_{2}x  + c_{1}x^{2} c_{3}x^{3}. 
\end{equation}
% 
\autoref{eq:cubiC} has four degrees of freedom and requires and requires a $4x4$ system of linear equations to compute the coefficients $c_{i}$, $i=0, \cdots, 3$. 
%
A common approach is to use the data and derivatives values a the edge nodes to build the system of linear equations and find the coefficients. 
% 
Let $(x_{i}, u_{i}, du_{i})$ and $(x_{i+1}, u_{i+1}, du_{i+1})$ the data values associated with the edge or interval $[x_{i}, x_{i+1}]$.
%
The coefficients are obtained by solving  
\begin{equation} 
\begin{pmatrix}
    q(x_{i}) =  u_{i} \\
    q(x_{i+1}) =  u_{i+1} \\
    q^{'}(x_{i}) =  du_{i+1} \\
    q^{'}(x_{i+1}) =  du_{i+1}
\end{pmatrix}
\end{equation}
%
The intersection is then obtained by finding the roots to the problem $q(x)=k$, where $k$ is the isovalue of interest.
%
We note that for many data sets the values of the derivatives are not available and are therefore approximated using finite difference methods.


\subsection{WENO Interpolation}
\label{subsec:weno}
%
The WENO method ~\cite{ZHANG2016103} is a high-order polynomial reconstruction method developed for solving hyperbolic and convection-diffusion equations.
%
WENO is an extension of the essentially non-oscillatory method ~\cite{Shu1989}.
%
WENO is a polynomial approximation procedure that achieves high-order accuracy in smooth regions and provides a better representation of regions with sharp gradients compared to traditional Lagrange interpolation.
%

Let's consider the  1D mesh defined as 
\begin{equation} \label{eq:mesh}
    \mathcal{M} = \{\cdots, x_{i-2}, x_{i-1}, x_{i}, x_{i+1}, x_{i+2}, x_{i+3}, \cdots \},
\end{equation}
where $i \in \mathbb{N} \cup \{0\}$, and $\{ \cdots, x_{i-2}, x_{i-1}, x_{i}, x_{i+1}, x_{i+2}, x_{i+3}, \cdots \}$, correspond to the data associated with the mesh $\mathcal{M}$.
%
For each interval $I_{i}$ or edge where the isovalue lies between $u_{i}$ and $u_{i+1}$, a high-order polynomial $p_{i}(x)$ is used to approximate the function inside the interval $I_{i}$.
%
The interpolant $p_{i}(x)$ is then used to form the implicit equation $p_{i}(x)- isovalue =0$ that is solved to find the intersection with the corresponding edge.

The final interpolant $p_{i}(x)$ is a convex combination of the third-order approximations $p^{(1)}(x)$, $p^{(3)}(x)$, and $p^{(3)}(x)$
\begin{equation}\label{eq:p_i}
    p_{i}(x) = w_{1}p^{(1)}(x) + w_{2}p^{(2)}(x) + w_{3}p^{(1)}(x), 
\end{equation}
where $w_{1}, w_{2}$, and $w_{3}$ are nonlinear weights such that $w_{1}+w_{2}+w_{3} =1$.
%
The nonlinear weights are obtained using the ``smoothness" indicator $\beta_{j}$ in ~\cite{Jiang1996} that can be approximated as follows:
%
\begin{equation}\label{eq:smoothness_indicators}
\begin{aligned}
    \beta_{1} = & \frac{13}{12} \big( u_{i-2} - 2u_{i-1} + u_{i}\big)^{2} + \frac{1}{4} \big( u_{i-2}-4u_{i-1}+ 3u_{i}\big)^{2}, \\
    %
    \beta_{2} = & \frac{13}{12} \big( u_{i-1} - 2u_{i} + u_{i+1}\big)^{2} + \frac{1}{4} \big( u_{i-1}-u_{i+1}\big)^{2}, \\
    %
    \beta_{3} = & \frac{13}{12} \big( u_{i} - 2u_{i+1} + u_{i+2}\big)^{2} + \frac{1}{4} \big( 3u_{i}-4u_{i+1}+ u_{i+2}\big)^{2}, \\
\end{aligned}
\end{equation}
%
The nonlinear weights are also dependent on the constants $\gamma_{j}$ for $j=1,2,3$.
\begin{equation} \label{eq:linear_weigts}
    \gamma_{1} = \frac{1}{10}, \quad \gamma_{2} = \frac{3}{5}, \quad \gamma_{3} = \frac{3}{10}.
\end{equation}
%
Using the ``smoothness" indicator in \autoref{eq:smoothness_indicators} and the constant weight in Equation \autoref{eq:linear_weigts}, the nonlinear weight can be expressed as follows:
\begin{equation}
    w_{j} = \frac{\alpha_{j}}{\alpha_{1}+\alpha_{2}+\alpha_{3}}, \quad \alpha_{j} = \frac{\gamma_{j}}{(\epsilon+\beta_{j})^{2}}, \quad j=1,2,3.
\end{equation}
%
The parameter $\epsilon$, typically set to $10^{-6}$, is introduced to avoid division by zero.
%
Jiang and Shu ~\cite{Jiang1996} proved that in smooth regions the approximation $p_{i}(x)$ in Equation (\ref{eq:p_i}) is fifth-order accurate.  

%
Solving the implicit equation $p_{i}(x)=isovalue$ is equivalent to a root-finding problem for a cubic polynomial.
%
%The roots for the WENO polynomial can be found using the cubic formula in ~\cite{weisstein2002}.
%
Similar to ~\cite{Fuhrmann2015} the median solution is selected in the cases where multiple valid roots are found.
%
Overall, the WENO method uses a convex combination of third-order (cubic) polynomials with nonlinear weights to achieve fifth-order accuracy. 



==> old/extras.tex <==
\section{Extras}

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.45 \textwidth}
    \centering
        \includegraphics[scale=0.15]{extras-figures/fig-tangle.png}
        \caption{}
        \label{}
    \end{subfigure}
    %%
    \begin{subfigure}[b]{0.45 \textwidth}
        \centering
        \includegraphics[scale=0.15]{extras-figures/fig-teardrop.png}
        \caption{}
        \label{}
    \end{subfigure}
    %%
    \caption{Linear Error}
    \label{fig:enter-label}
\end{figure}


==> old/methods.tex <==

\section{Method}
\label{sec:method}

Here, we introduce the different methods for visualizing and analyzing isosurfaces obtained from the MC algorithms. 


\subsection{Error Approximation}
\label{subsec:error_approximation}
    %
    We propose an edge-crossing error approximation for MC algorithms that is derived from linear polynomial error.
    %
    This approximated error is used to visualize and explore the isosurface uncertainty from the linear interpolation model in the MC algorithm.   
    %
    Let the $\ell(x)$ be the linear approximation of the underlying function $f(x)$ for $x \in [x_{i}, x_{i+1}]$.
    %
    The interpolation error from the linear polynomial approximation is
    %
    \begin{align}\label{eq:error}
        e(x) =  \ell(x) - f(x) = \frac{f^{''}(\xi)}{2}(x-x_{i})(x-x_{i+1}),
    \end{align}
    %
    where $\xi \in (x_{i-1}, x_{i+2})$.
    MC algorithms approximate the underlying function $f(x)$ with the linear polynomial $\ell(x)$ and solve implicit problem $\ell(x)=k$ where $k \in \mathbb{R}$ is the isovalue.
    %
    Let $x_{*}$ and $\bar{x}_{*}$ the solutions to $\ell(x)=k$ and $f(x)=k$, respectively.
    %
    The Newton polynomial presentation of $\ell(\bar{x}_{*})=k$ can be written as 
    %
    \begin{align}\label{eq:l_of_x}
        f(x_{i})+U[x_{i}, x_{i+1}] (\bar{x}_{*}-x_{i}) + \frac{f^{''}(\xi)}{2}(\bar{x}_{*}-x_{i})(\bar{x}_{*}-x_{i+1}) = c
    \end{align}
    %
    where $U[i, i+1]$ is divided differences obtained from the general recursive expression
    %
    \begin{equation}
        \begin{gathered}
        U[i] = u_{i} = f(x_{i}), \quad U[i,i+1] = \frac{U[i+1] -U[i]}{x_{i+1} - x_{i}}, \\
        U[i, i+j] = \frac{U[i+1, \cdots, i+j]- U[i, \cdots, i+j-1]}{x_{i+j}-x_{i}},    
        \end{gathered}
    \end{equation}
    with $j$ being an integer.
    %
    Using \autoref{eq:error} and $\ell(x)$ in \autoref{eq:l_of_x}, the implicit function $f(x) = c$ can be explicitly expressed as follows:
    %
    \begin{align}\label{eq:f_of_x}
        f(x) = f(x_{i})+U[x_{i}, x_{i+1}] (x_{*}-x_{i}) + \frac{f^{''}(\xi)}{2}(x_{*}-x_{i})(x_{*}-x_{i+1}) = c
    \end{align}
    %
    Subtracting \autoref{eq:l_of_x} from \autoref{eq:f_of_x} we obtain the edge-crossing approximation error 
    \begin{align}
        |x_{*}-\bar{x}_{*}| = \Big|\frac{1}{U[x_{i}, x_{i+1}]}\frac{f^{''}(\xi)}{2} (x_{*}-x_{i})(x_{*}-x_{i+1}) \Big|.
    \end{align}
    %
    The edge-crossing approximation error can be bounded by 
    \begin{align}
        |x_{*}-\bar{x}_{*}| \leq \frac{\max_{\xi \in[x_{i}, x_{i+1}]} |f^{''}(\xi)|}{2U[i, i+1]}(x_{*}-x_{i})(x_{*}-x_{i+1})
    \end{align}
    In practice, $\frac{f^{''}(\xi)}{2}$, is approximated because $\xi$ and $f^{''}$ are not available.
    %
    \color{black}
    We approximate the vertex approximation error as follows:
    \begin{align}\label{eq:approx_linear_error}
        |x_{*}-\bar{x}_{*}| \approx \bar{e} = \frac{max\big( |U[i-1, i+1]|, |U[i, i+2]|     \Big)}{U[i, i+1]}(\bar{x}_{*}-x_{i})* (\bar{x}_{*}-x_{i+1}) 
    \end{align}
    %
    \autoref{subfig:vertex-error-illustration} shows the difference between the underlying function and the linear approximation.
    %
    \autoref{subfig:vertex-error} shows approximated error from \autoref{eq:approx_linear_error} and \autoref{subfig:metro-error} show computed error use Metro.
    %
    The error visualization from \autoref{subfig:vertex-error} and \autoref{subfig:metro-error} have similar patterns which demonstrate that the vertex approximation error provides a good estimate of isosurface uncertainty from using linear interpolation.
    
    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.30 \textwidth }
            \includegraphics[scale=0.20]{illustration/Vertex-error.png}
            \caption{Vertex error}
            \label{subfig:vertex-error-illustration}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth }
            \includegraphics[scale=0.30]{illustration/vertex-error-validation.png}
            \caption{Vertex error}
            \label{subfig:vertex-error}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth }
            \includegraphics[scale=0.30]{illustration/vertex-error-validation.png}
            \caption{error}
            \label{subfig:metro-error}
        \end{subfigure}
        %
        \caption{\autoref{subfig:vertex-error-illustration} shows the error for using linear interpolation in MC to extract a level-crossing at an edge. \autoref{subfig:vertex-error} shows isosurface error visualization from \autoref{eq:approx_linear_error}. \autoref{subfig:metro-error} shows the calculated error from Metro.}
        \label{fig:vertex-error}
    \end{figure}

    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/tangle_512x512x512_32x32x32.png}
            \caption{Error ($32^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/tangle_512x512x512_64x64x64.png}
            \caption{Error ($64^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/tangle_512x512x512_128x128x128.png}
            \caption{Error ($128^{3}$)}
            \label{}
        \end{subfigure}
        %%%
        %%%
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/tangle_Aprox_Err_32x32x32.png}
            \caption{ Approx. Error ($32^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/tangle_Aprox_Err_64x64x64.png}
            \caption{Approx. Error ($64^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/tangle_Aprox_Err_128x128x128.png}
            \caption{Approx. Error ($128^{3}$)}
            \label{}
        \end{subfigure}
        \caption{Tangle Example}
        \label{fig:enter-label}
    \end{figure}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/marschnerlobb_512x512x512_32x32x32.png}
            \caption{Error ($32^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/marschnerlobb_512x512x512_64x64x64.png}
            \caption{Error ($64^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/marschnerlobb_512x512x512_128x128x128.png}
            \caption{Error ($128^{3}$)}
            \label{}
        \end{subfigure}
        %%%
        %%%
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/marschnerlobb_Aprox_Err_32x32x32.png}
            \caption{ Approx. Error ($32^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/marschnerlobb_Aprox_Err_64x64x64.png}
            \caption{Approx. Error ($64^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/marschnerlobb_Aprox_Err_128x128x128.png}
            \caption{Approx. Error ($128^{3}$)}
            \label{}
        \end{subfigure}
        \caption{Marschner and Lobb Example}
        \label{fig:enter-label}
    \end{figure}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/teardrop_512x512x512_32x32x32.png}
            \caption{Error ($32^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/teardrop_512x512x512_64x64x64.png}
            \caption{Error ($64^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/teardrop_512x512x512_128x128x128.png}
            \caption{Error ($128^{3}$)}
            \label{}
        \end{subfigure}
        %%%
        %%%
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/teardrop_Aprox_Err_32x32x32.png}
            \caption{ Approx. Error ($32^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/teardrop_Aprox_Err_64x64x64.png}
            \caption{Approx. Error ($64^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.15]{figures/teardrop_Aprox_Err_128x128x128.png}
            \caption{Approx. Error ($128^{3}$)}
            \label{}
        \end{subfigure}
        \caption{Tear drop Example}
        \label{fig:enter-label}
    \end{figure}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/diamond_512x512x512_32x32x32.png}
            \caption{Error ($32^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/diamond_512x512x512_64x64x64.png}
            \caption{Error ($64^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/diamond_512x512x512_128x128x128.png}
            \caption{Error ($128^{3}$)}
            \label{}
        \end{subfigure}
        %%%
        %%%
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/diamond_512x512x512_32x32x32.png}
            \caption{ Approx. Error ($32^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/diamond_Aprox_Err_64x64x64.png}
            \caption{Approx. Error ($64^{3}$)}
            \label{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.30 \textwidth}
            \includegraphics[scale=0.12]{figures/diamond_Aprox_Err_128x128x128.png}
            \caption{Approx. Error ($128^{3}$)}
            \label{}
        \end{subfigure}
        \caption{Absolute Value Example}
        \label{fig:enter-label}
    \end{figure}



    \subsection{Hidden Features Recovery}
    \label{subsec:hidden_features}
    %
    The MC algorithms with and without sharp feature recovery fail to identify and reconstruct hidden features that are not captured by the mesh resolution. 
    %
    These hidden features are isosurface patches not detected by linear interpolation and the topological case considered in MC algorithms. 
    %
    The hidden features alter the isosurface connectivity and its overall structure.
    %
    We propose a novel method for hidden feature detection and recovery that relies on the slopes (divided differences) on cell edges and high-order interpolation.
    
    \begin{itemize}
        \item  A cell might have a hidden feature if for any of its edges two of the three slopes $U[i-1, i]$, $U[i, i+1]$, and $U[i, i-1]$ of neighboring edges have opposite signs. 
        \item The detected cell is divided into smaller subcells using tri-cubic Lagrange polynomial interpolation. We note that using linear interpolation instead for the cell refinement doesn’t recover the missing hidden features. The first derivatives at the subcell nodes are approximated using the derivative of the tri-cubic interpolant.
        \item The MC algorithm with cubic interpolation is then applied to each subcell to reconstruct the hidden features.
    \end{itemize}

    %
    \autoref{fig:hidden_feature_illustrations1} shows a 1D example where the vertex crossings on the middle edge are detected using the slopes (divided differences) of the neighboring edges.
    %
    The middle edge is split into two new edges that can then be used to detect and approximate the edge crossing.
    %
    The scalar value at the split location is obtained using cubic interpolation.
    %
    \autoref{fig:hidden_feature_illustrations2} provides an illustration using a marching square in the 2D case.
    %
    The MC algorithms with and without sharp feature-preserving methods don't recover the hidden feature in blue. 
    %
    This cell is considered above the desired isoline because all its node values are larger than the target isovalue. 
    %
    The cell outlined with black lines is divided into smaller cells, indicated by the dashed lines, using tri-cubic interpolation.
    %
    These new cells reveal new edge crossings that can be used to represent the hidden feature and better approximate the overall isosurface.
   
    %
    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.45 \textwidth}
            \includegraphics[scale=0.40]{illustration/sharp-feature.png}
            \caption{}
            \label{fig:hidden_feature_illustrations1}    
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.40 \textwidth}
            \includegraphics[scale=0.40]{figs/hidden-feature-illustration.png}
            \caption{}
            \label{fig:hidden_feature_illustrations2}    
        \end{subfigure}
        \caption{}
        \label{fig:hidden_feature_illustrations}
    \end{figure}
   
    These cell refinements lead to cracks in the reconstructed isosurface.
    %
    We resolve this issue by connecting the edges at hidden feature boundaries with edges at the boundaries of the reaming isosurface.
    %
    The cells at the boundaries of the isosurface with no hidden features are modified during the polygon extraction to ensure a crack-free isosurface.

    MAYBE ILLUSTRATION FIGURE

\subsection{Visualization and Analysis of Isosurface uncertainty}
    
 \newpage
    \subsection{Adaptive Refinement}
    \label{subsec:adaptive_refinement}
    %% Introduction
    Traditional MC algorithms fail to recover sharp features that are not captured by the mesh resolution.
    %
    The feature-preserving methods are based on sampling normals on the cell edges and inserting more points in the surface triangulation to better capture the hidden features.
    %
    The process of inserting more points can be done via adaptive refinement which is the approach adopted in this work.
    %
    We note that in practice, finer resolution datasets and normals on the interior of edges are not often available.
    %
    The normals on the interior of the edges are typically approximated by first using centered finite difference to approximate derivates and normals of the edge endpoints and then linearly interpolating those normals to the interior of the edge.
    %
    For edges with large gradients center difference can lead to large errors and linear interpolation assumes that normals and derivatives are monotonic over the edge length.

    We overcome these limitations by using the divided differences from the neighboring cells to detect the sharp features, and the target cell is subdivided using cubic and WENO interpolation.
    %
    We assume that a cell has a sharp feature if for any of its edges two of the three $u[i-1, i]$, $U[i,i+1]$, and $U[i+1, i+2]$, divided differences of the neighborhood intervals have opposite signs.  
    %
    The cubic or WENO interpolation applied successively to the x, y, and z axes is used to subdivide the target cell to better capture the sharp feature. 
    %

    
    %
    \autoref{fig:hidden_feature_illustrations1} shows an example where the hidden feature is detected using the divided differences an underlying function is approximated using a polynomial.
    %
    Once the edge is subdived the MC algorithm with cubic or WENO can be used to extract more accurate level-crossing and better present the sharp feature.
    \autoref{fig:hidden_feature_illustrations2} provides an illustration using a marching square in the 2D case.
    %
    Adaptively refining the cell leads to a more accurate approximation of the hidden feature as demonstrated in \autoref{fig:hidden_feature_illustrations2}. 
    %
    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.45 \textwidth}
            \includegraphics[scale=0.40]{illustration/sharp-feature.png}
            \caption{}
            \label{fig:hidden_feature_illustrations1}    
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.45 \textwidth}
            \includegraphics[scale=0.40]{illustration/Amr-2d.png}
            \caption{}
            \label{fig:hidden_feature_illustrations2}    
        \end{subfigure}
        \caption{}
        \label{fig:hidden_feature_illustrations}
    \end{figure}

    
    \color{blue}
    HOW DO WE HANDLE CRACKS
    \color{black}
   
    %\begin{figure}[H]
    %    \centering
    %    \begin{subfigure}[b]{0.48 \textwidth}
    %        \includegraphics[scale=0.35]{figures/illustration01.eps}
    %        \caption{}
    %        \label{}
    %    \end{subfigure}
    %    %
    %    \begin{subfigure}[b]{0.48 \textwidth}
    %        \includegraphics[scale=0.35]{figures/illustration02.eps}
    %        \caption{}
    %    \end{subfigure}
    %    %
    %    \caption{Caption}
    %    \label{fig:enter-label}
    %\end{figure}


    \subsection{Adaptive Interpolation}
    \label{subsec:adaptive_interpolation}
    %% Problem
    The traditional MC algorithm based on linear interpolation, although fast and local, can introduce significant errors and undesirable visual artifacts and degrade the isosurface approximation [6, 7].
    %
    Using quadratic [REF] and cubic [REF] interpolation methods can improve the approximation and reduce the visual artifacts.
    %
    The quadratic and cubic polynomials have an $O(h^{3})$ and $O(h^{4})$ order of accuracy, respectively.
    %
    In addition, the cubic interpolation methods require the approximation of the first derivatives at the cell nodes. 
    %
    This approximation is typically done using center difference stencil which can lead to large errors in cases with sharp gradient and $C^{0}$-continuities, as shown in \autoref{fig:HO-fail}
    %
    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.45 \textwidth}
            \includegraphics[scale=0.3]{illustration/HO-fail1.png}
            \caption{}
            \label{subfig:HO-fail1}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.45 \textwidth}
            \includegraphics[scale=0.3]{illustration/HO-fail2.png}
            \caption{}
            \label{subfig:HO-fail2}
        \end{subfigure}
        \caption{Caption}
        \label{fig:HO-fail}
    \end{figure}

    %% Solution to problem
    To overcome these limitations, we propose an adaptive polynomial approximation method.
    %
    This method provides the flexibility to adaptively select the polynomial interpolation technique to use based on (1) and user-specified vertex approximation error threshold and the characteristics of the different intervals, and (2) user-specified regions where to apply the different interpolation methods.
    %
    \subsubsection*{Threshold Based Adaptive Interpolation}
        In this approach, The characteristics of the different intervals/regions are determined using the vertex approximation error from linear interpolation introduced in the previous \autoref{subsec:adaptive_interpolation} and the divided differences.
        %% Solution in non-smooth regions
        \autoref{fig:HO-fail} shows that inside a region with sharp gradients or where the underlying function is linear, the polynomial interpolation error and the divided-differences $U[i,+1]$, $U[i, i+2]$, and $U[i-1, i+1]$ has small values that are close to zero.
        %
        At the boundaries of regions with sharp gradients, high-order polynomial approximation leads to large errors and divided differences, as demonstrated in Figure [REF].
        %
        In these regions, linear interpolation is better suited for approximating the underlying function compared to typical cubic interpolation.
        %
        To further improve the accuracy, we propose the ENO method.
        %
        In addition to providing a better approximation in non-smooth regions, the ENO method has a higher order of accuracy $O(h^{4})$ compared to linear ($O(h^{2})$).  
        %

        %% Solution in smooth regions
        Using cubic interpolation in remaining smooth regions leads to more accurate polynomial approximation and therefore better surface reconstructions compared to linear interpolation.
        %
        We propose the WENO method to further improve the accuracy in these smooth regions. 
        %
        The WENO method has higher order of accuracy ($O(h^{5})$) compared to the typical cubic interpolation methods ($O(h^{4})$).
        %
        As in the typical cubic interpolation, the high order accuracy of the WENO method breaks down in regions with sharp gradients, discontinuities, and $C^{0}$-continuities. 

    \subsubsection*{Region-Specific Adaptive Interpolation}
        %
        In this approach, the user specifies the regions where to apply the different interpolation methods.
        %
        The selection of the region and interpolation techniques are informed by prior knowledge of the underlying data, linear approximation errors from \autoref{subsec:adaptive_interpolation},  and exploration of the surface features and uncertainty.
        %
        In many simulations, one is often interested in visualizing and exploring the region containing the properties or features of interest most. 

        \autoref{fig:HO-all} shows an example where linear, cubic, and WENO are applied to the selected region in [color]. 
        %
        This example demonstrates that cubic and WENO improve the isosurface accuracy in the selected region, and provide a comparison between linear, cubic, and WENO interpolation methods.

        \begin{figure}
            \centering
            \begin{subfigure}[b]{0.20 \textwidth}
                \includegraphics[scale=0.18]{illustration/HO-all.png}
                \caption{}
                \label{subfig:HO-all}
            \end{subfigure}
            %
            \begin{subfigure}[b]{0.20 \textwidth}
                \includegraphics[scale=0.14]{illustration/HO-L.png}
                \caption{}
                \label{subfig:HO-L}
            \end{subfigure}
            %
            \begin{subfigure}[b]{0.20 \textwidth}
                \includegraphics[scale=0.14]{illustration/HO-C.png}
                \caption{}
                \label{subfig:HO-C}
            \end{subfigure}
            %
            \begin{subfigure}[b]{0.20 \textwidth}
                \includegraphics[scale=0.14]{illustration/HO-W.png}
                \caption{}
                \label{subfig:HO-W}
            \end{subfigure}
            \caption{Caption}
            \label{fig:HO-all}
        \end{figure}
        
    \subsection{Isosurface Analysis and Visualization Framework}
        %% small intro
        Here, we introduce a unifying framework for visualizing and analyzing surface uncertainty under local adaptive refinement and different interpolation methods. 
        %
        Often isosurface visualization does not provide any insight into the uncertainty of surface reconstruction error let alone the uncertainty and variability from using different interpolation models. 
        %
        This framework employs the previous ideas introduced in \autoref{subsec:error_approximation}, \autoref{subsec:adaptive_refinement}, and \autoref{subsec:adaptive_interpolation} to enable visual analysis of surfaces obtained from using different interpolation methods.

        %% Visualization linear interpolation 
        %% visualization of hidden features
        This framework provides a visualization of the surface obtained from the traditional MC algorithm with linear interpolation and overlaid with the vertex approximation error at each triangle node, as shown in Figure [REF].
        %
        In addition, Figure [REF] demonstrates that the surface can be used to highlight the cells with sharp features. 
        %
        These surface visualizations coupled with error approximation and sharp features highlighting give insight into uncertainties and limitations of linear interpolation for a given isosurface.
        %
        This information can be used to guide the adaptive refinement and interpolation to improve the quality of the surface and/or target specific regions to explore a compare the differences between interpolation methods. 

        \begin{figure}
            \centering
            \begin{subfigure}[b]{0.45 \textwidth}
                \includegraphics[scale=0.4]{illustration/vertex-error-validation.png}
                \caption{}
                \label{subfig:vertex-error2}
            \end{subfigure}
            %
            \begin{subfigure}[b]{0.45 \textwidth}
                \includegraphics[scale=0.4]{illustration/vertex-sharp-feature.png}
                \caption{}
                \label{subfig:sharp-feature}
            \end{subfigure}
            %
            \caption{Caption}
            \label{fig:}
        \end{figure}

       
        %% user-specified adaptive interpolation methods
        [Framework Name] allows the user to select one or two interpolation techniques between linear, cubic, and WENO methods and choose where and how to apply the selected interpolation method.
        %
        The same interpolation method is applied to the entire domain when a single interpolation technique is selected.
        %
        In the case of two interpolation techniques, a vertex approximation error threshold can be specified to guide how the adaptive interpolation is applied.
        %
        In the intervals where the error is above the indicated threshold, a cubic or WENO interpolation is used. 
        %
        Alternatively, the user can directly specify the region where to use the cubic or WENO interpolation.
        %
        a linear or ENO interpolation is used inside the remaining intervals or regions.
        %
        
        %user-specified adaptive refinement 
        Adaptive refinement can be employed to improve and evaluate the quality of the reconstructed surface.
        %
        This work provides two options for refinement. 
        %
        The first refines the cells with hidden features and the second refines a selected domain.
        %
        The option to use can be indicated by using the parameter [xyz] in the framework interface.
        %


        %% Visualization of surface differences based on using different interpolation methods
        %% Topological visualization of surface features (critical points)
        In [the bottom left] of the framework interface, we compare the differences between the surfaces and surface features obtained from the different interpolation models. 
        %
        This enables visual analysis of the surface variability from using adaptive refinement and different interpolation models in specific intervals or regions of interest.
        %
        For example, Figure [REF] shows the difference between [xyz]and [xyz].
        %
        Furthermore, we visually compare and evaluate the surface features or topology obtained from the different interpolations.
        %
        Overall, the various features and visualization in [Framework Name] highlight the uncertainties and limitations associated with using linear interpolation in MC-type algorithms and provide a flexible way of comparing and analyzing the differences between the surfaces obtained from several configurations.
        %
        These configurations include using vertex approximation errors, different adaptive and non-adaptive interpolation methods, and adaptive refinement. 

        %% Interface description
        \begin{figure}[H]
            \centering
            \includegraphics[scale=0.6]{illustration/frame-work.png}
            \caption{Caption}
            \label{fig:frame-work}
        \end{figure}

        



==> old/outline-old.tex <==
\section{}

\section{Introduction}
%
Contributions:
\begin{itemize}
    \item Identify hidden isovalue vertices missed by linear interpolation approach
    \item Adaptive WENO for more accurate interpolation and triangulation (WENO + ENO)
    \item Robustness analysis of L, C, WENO and AWENO
\end{itemize}

\section{Related Work}

\section{Background}
%
    \subsection{Marching Cube}
    %
    \subsection{Linear Interpolation}
    %
    \subsection{Cubic Interpolation}
    %
    \subsection{WENO Interpolation}
    %

\section{Methods}
%
    \begin{itemize}
        \item Limitations of Linear Interpolation
            \begin{itemize}
                \item Not accurate 
                \item introduce artifacts
                \item no suitable for handling hidden extrema 
            \end{itemize}
        \item Benefits and limitation of Cubic and WENO
            \begin{itemize}
                \item Improve accuracy 
                \item help reduces artifacts from Linear interpolation
                \item Not accurate for discontinuities, C0-continuities, and steep gradients
                \item More expensive than Linear interpolation 
            \end{itemize}
        \item Benefits and limitation of AWENO
            \begin{itemize}
                \item Benefit from high order accuracy from WENO in smooth regions $O^{h^{5}}$ and ENO in nonsmooth regions $O(h^{4})$
                \item provide a better approximation of  discontinuities, C0-continuities, and steep gradients compared to L, C, W
                \item suitable for handling hidden extrema
                \item more expensive than linear interpolation
            \end{itemize}
    \end{itemize}

    
    \begin{figure}[H]
        \centering
        \begin{subfigure}[b]{0.48 \textwidth}
            \includegraphics[scale=0.35]{figures/illustration01.eps}
            \caption{}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.48 \textwidth}
            \includegraphics[scale=0.35]{figures/illustration02.eps}
            \caption{}
        \end{subfigure}
        %
        \caption{Caption}
        \label{fig:enter-label}
    \end{figure}

    \subsection{Edge with Hidden Isovalue}
    %
    \subsection{Adaptive WENO}
    %
    \subsection{Isosurface Variability for the Interpolation Methods}

%

\section{Results}
%
    \begin{itemize}
        \item Examples demonstrating limitations of Linear, Cubic, and WENO 
        \item Examples demonstrating superior accuracy of Aadaptive WENO $O(h^{5})$ compared to Cubic $O(h^{4})$ and linear $O(h^{2})$
        \item Example demonstrating artifacts from linear interpolation
        \item example demonstrating better surface reconstrcution when incorporating edeges with hidden isovalue
        \item Example demonstrating that AWENO help remove artifacts and compare against Cubic and WENO
    \end{itemize}

\section{Discussion}
\begin{itemize}
    \item summary of the methods
    \item summary of the results
    \item benefits and limitation of AWENO
\end{itemize}
\section{Conclusion}
%
\begin{itemize}
    \item summary of contributions
    \item potential furtur reseach directions
\end{itemize}


==> old/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
%
The marching cubes ~\cite{Willam1987} algorithm is the most popular method for surface extraction and visualization from 3D hexahedral mesh data.
%
For each hexahedral cell, the algorithm uses linear interpolation to extract the corresponding approximation of the surface in the cell.
%
Several variants of the MC algorithm have been developed to resolve ambiguous cases ~\cite{Nielson1991, Lewiner2003, Claudia1994} and extend the algorithm to nonuniform structured meshes ~\cite{SCI:She95a, Michael2007, Bloomenthal19883, Gokul2004}.

\subsection{Isosurface Uncertainty}
%Uncertainty vis for isosurface
Estimating and visualizing isosurface uncertainty is a challenging problem [REFS].
%
One typically considers the uncertainty originating from noisy data and/or from different isosurface extraction and visualization models.
%
The former is the most common approach used for estimating and visualizing isosurface uncertainties \cite{Pfaffelmoser2011, Pothkow2011_1, Pothkow2013, Athawale2013, Athawale2016, Athawale2021, Rhodes2003}.
%
This study focuses on the model uncertainty in MC algorithms which is highly unexplored.
%
More specifically, we study the isosurface errors/variations obtained from using interpolation methods in MC-type algorithms. 
%
Before diving into the details of this study, we highlight several related works focused on isosurface uncertainty.

Several statistical approaches based on parametric \cite{Athawale2013} and nonparametric models \cite{Pothkow2013, Athawale2016} have been introduced to quantify and visualize isosurface uncertainty from ensemble data.
%
These statistical methods provide measure metrics such as mean and variance that can be used to visualize the most probable isosurface and its uncertainty.
%
For instance, Athawale et al. provided a closed form for computing the expected position and variance of the level-crossing in the MC algorithm for parametric \cite{Athawale2013} and nonparametric \cite{Athawale2016} distributions. 
%
Topology case count and entropy-based methods can be used to resolve ambiguity in MC algorithm and visualize isosurface uncertainty \cite{Athawale2021}.
%
The satirical approaches often require the use of sampling methods such as Mote Carlo sampling which are computationally expensive.
%
Though the closed forms in \cite{Athawale2013, Athawale2016, Athawale2021} improve the performance for independent noise models, they are not available for other more complex noise models such as multivariate Gaussian assumption.
%
To address the performance limitations Han et al. \cite{Han2022} use deep learning to accelerate level-set uncertainty computation under Gaussian noise assumption; and Wang et al. \cite{Wang2023} leverage the parallelism and portability from VTK-m to accelerate the uncertainty computation and visualization in the Filter for uncertainty visualization of Marching Cubes on Multi-Core devices ($FunMC^{2}$).



In the context of multiresolution data Rhodes et al. \cite{Rhodes2003} the use of color and texture to visualize the isosurface uncertainty. 
%
The surface error is obtained by linear interpolation of the volume data errors to vertices during the isosurface extraction process. This work focuses on the error between coarse and finer mesh data. 



%Kamal et al. \cite{Kamal2021} Survey

%Pfaffelmoser et al. \cite{Pfaffelmoser2011} Statical modeling of data uncertainty.
%
%A measure for estimating the distance between possible isosurface variations and the mean surface are introduced and used to improve the visualization of isosurface variability.


%P\"{o}thkow and Hege \cite{Pothkow2013} propose nonparametric models for estimating and visualizing uncertainty from ensemble data.

\subsection{Interpolation in MC}
%
It is well established that the linear interpolation method in the MC algorithm can lead to large approximation errors and undesirable artifacts.
%
To address this limitation, several studies have explored the use of high-order interpolation methods for more accurate isosurface approximation ~\cite{Fuhrmann2015, Balazs2019, Cohen-Or2000}.
%

%
Fuhrmann et al. ~\cite{Fuhrmann2015} have developed Hermite quadratic and cubic interpolation techniques for isosurface constructions. 
%
The Hermite interpolation methods are used to approximate the isovertex on each edge. 
%
Fuhrmann et al. ~\cite{Fuhrmann2015} compares these methods against linear interpolation using synthetic and real-world datasets. 
%
These approaches require the values of the first derivative of the mesh point, which can be approximated using finite difference methods.
%
Standard rendering uses linear interpolation to reconstruct the underlying profile from data and estimate the gradients for the shading computation.
%
Cs\'{e}bfalvi, Bal\'{a}zs ~\cite{Balazs2019} demonstrated that the same sampling points used for shading can be employed to build cubic interpolants without incurring additional storage and rendering costs while benefiting from the high-order interpolation compared to linear interpolation.
%
The reconstructed cubic interpolant is equivalent to the Catmull-Rom spline kernel.
%
Lin et al. ~\cite{Lin2021} have introduced a refactoring of quadratic and cubic interpolation based on the structure of linear interpolation to improve performance over the traditional high-order interpolation methods.
%
In addition to the performance gain, high-order interpolation can be performed adaptively by skipping high-order terms with small coefficients.
%
Zhang et al. ~\cite{Zhang2022} have improved surface reconstruction by accelerating evaluation speed using signed marching cubes.
%
Their method has two steps and is based on a fast multipole method.
%
The first step consists of using the fast multipole method with low order to evaluate all points of the voxels and identify the voxels that intersect with the isosurface.
%
The second step uses the fast multipole method with high order to evaluate the points of the intersecting voxels and construct the isosurface.

%Most of the high-order interpolation methods used in the MC-type methods are based on cubic polynomials that are third-order accurate.
%%
%In addition, these polynomials are not bounded and may lead to undesirable oscillations.
%%
%This work presents high-order WENO and AWENO interpolation methods for MC-type methods.
%%
%Both methods are based on WENO interpolants, which are fifth-order accurate.

\subsection{Sharp Features}
% Adaptive refinement for feature detection

The traditional MC algorithms fail to recover sharp features that are not captured by mesh resolution.
%
Several studies have extended the MC algorithms to incorporate feature-preserving techniques that can recover these sharp features \cite{Kobbelt2001, Ju2002, Ho2004, Ho2005, NEWMAN2006, YU2008, Dietrich2009, BAGLEY2016}.
%
These methods use information about the cell derivatives to better represent the underlying sharp features.
%
Recently, machine learning-based approaches have been proposed for more accurate MC with feature preservation \cite{Chen2021, FENG2023, Chen2022, Remelli2020, Gao2020}.


Kobelt et al \cite{Kobbelt2001} propose a surface extraction method from directed distance field and surface normals of a geometric object that preserves sharp features.
%
The normals are used to detect the sharp features and new sample points are added inside the cell to recover the hidden features.
%
The Dual contouring algorithm proposed in \cite{Ju2002} uses the edges intersection and the normals at those intersections to process the cells with sharp features.
%
This method doesn't explicitly require identifying the cell with sharp features because it uses a quadratic error function to automatically place the additional points that are used to better represent the features.
%
Ho et al. \cite{Ho2005} propose to sample the edges normals to detect the cell with sharp features in volumetric data. 
%
These cells are then subdivided the better represent the sharp features. 
% 
The adaptive refinement of the cell requires access to a finer-resolution version of the data.


%
These techniques for hidden feature recovery require access to a finer resolution version of the input data to both detect and subdivide the target cells.
%
In many practical real-world examples, finer-resolution data are often not available. 
%
We propose to employ the local neighboring cells to identify the target cell with hidden features and construct a polynomial approximation that can then be used to subdivide the cell.
%



==> old/results.tex <==
\section{Results}
This Section provides several examples used to evaluate the visualization framework, interpolation methods, and feature-preserving technique for isocontour and isosurface extraction from 2D and 3D data.
%
Synthetic and real-world datasets are used to compare and evaluate the accuracy of the different approaches described in \autoref{sec:method}.
%
In the examples below, we measure the errors or distances/differences between two surfaces using the measuring error on simplified surfaces (METRO) ~\cite{Cignoni1998} tool.
%
The letters L, C, W are used to represent linear, cubic, WENO, respectively.
%
The adaptive interpolation method is represented using 2 letters. 
%
For example, if the interpolation method uses linear and WENO it is represented with L+W.
%

\subsection{Limitation of Linear Interpolation}
%
[framework Name] highlights the uncertainty associated with using linear interpolation in MC algorithms on [dataset name] with the isovalue set to [xyz].
%
The level-crossing approximated errors are calculated using [Equation xyz].
%
\autoref{subfig:vertex-error-linear} and \autoref{subfig:vertex-error-true} show the vertex (level-crossing) approximation errors and the errors obtained from computing the difference between the extracted and target isosurfaces, respectively.
%
The cell with sharp features are detected by comparing the neighborhood divided difference of the edeges
in each cell.
%
\autoref{subfig:vertex-sharp-features} highlights the cells with sharp features that are not captured by the traditional MC algorithm.
%
The first part of [framework name] is designed to visually reveal the limitations of using linear interpolation in MC algorithms.
%
\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/vertex-error-validation.png}
        \caption{Vertex error}
        \label{subfig:vertex-error-linear}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/vertex-error-validation.png}
        \caption{Error}
        \label{subfig:vertex-error-true}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/vertex-sharp-feature.png}
        \caption{Sharp Features}
        \label{subfig:vertex-sharp-features}
    \end{subfigure}
    
    \caption{Caption}
    \label{fig:linear-limitations}
\end{figure}


\autoref{subfig:features_linear} demonstrates that the sharp features can be recovered by refining the cells identified in \autoref{subfig:vertex-sharp-features} and using MC algorithms.
%
The accuracy of the isosurface can be further improved by the cubic or WENO interpolation, as shown in \autoref{subfig:features_cubic} and \autoref{subfig:features_weno}.
%
The cubic and WENO provide a more accurate approximation of the level-crossing for each cell.
%
\autoref{subfig:features_weno} also shows that WENO leads to smaller errors compared to cubic and linear.
%
\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/place_holder.png}
        \caption{Feature + Linear}
        \label{subfig:features_linear}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/place_holder.png}
        \caption{Feature + Cubic}
        \label{subfig:features_cubic}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/place_holder.png}
        \caption{Feature + WENO}
        \label{subfig:features_weno}
    \end{subfigure}
    \caption{Caption}
    \label{fig:improved_accuracy}
\end{figure}

\subsection{Adaptive Interpolation}
%
In many application, one is primarily interested in the quality of the isosruface reconstruction in specific local regions. 
%
These local regions are know apriori or identified the user when exploring the data.
%
For examples, the regions with the target features or large level-crossing errors can be considered.
%
In addition, using high-order interpolation without consideration of the underlying function behavior can lead to large errors in regions with large gradients and $C^{0}$-continuity.
%
The cubic and WENO interpolation methods require access to the neighboring cells and are computationally more expensive than line interpolation which local and fast.
%
Thus, using an adaptive interpolation method where the cubic or WENO method is only used inside a small region and linear in the remaining regions is computationally cheaper than using cubic or WENO for all the active cells.


[Figure] Shows the isosurface errors when using the WENO and cubic interpolation method.
%
The [datset name] has [large gradients and $C^{0}$-continuities] that are difficult to recover using cubic or WENO.
%
These [large gradients and $C^{0}$-continuities] can be represented using linear or ENO, as shown in [Figure].
%
However, using linear interpolation or ENO, which are $O(h^2)$ and $O(h^4)$, decreased the isosurface accuracy in the smooth regions because they have a low order of accuracy compared to WENO which is $O(h^{5})$.
%
[Figure] shows that this issue can be addressed using an adaptive interpolation method.
%
The adaptive interpolation uses linear or ENO in the regions with [large gradients and $C^{0}$-continuities] and cubic or WENO in the remaining.
%

[Figure], shows and example where the cubic or WENO is applied inside the specified region. 
%
In this example the specified region corresponds where the [linear interpolation has large errors].
%
[Figures] show isosurface results using L, L+C, L+W. 
%
The errors in the selected region decreases with using the higher order interpolants.
%

%
\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/place_holder.png}
        \caption{Linear}
        \label{subfig:linear}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/place_holder.png}
        \caption{Cubic}
        \label{subfig:cubic}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/place_holder.png}
        \caption{WENO}
        \label{subfig:weno}
    \end{subfigure}
    %
     \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/place_holder.png}
        \caption{L+C}
        \label{subfig:example_LC}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/place_holder.png}
        \caption{L+W}
        \label{subfig:example_LW}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3 \textwidth}
        \includegraphics[scale=0.3]{illustration/place_holder.png}
        \caption{E+W}
        \label{subfig:example_EW}
    \end{subfigure}
    \caption{Caption}
    \label{fig:adaptive_interpolation}
\end{figure}

  \begin{figure}[H]
            \centering
            \begin{subfigure}[b]{0.20 \textwidth}
                \includegraphics[scale=0.18]{illustration/HO-all.png}
                \caption{}
                \label{subfig:HO-all2}
            \end{subfigure}
            %
            \begin{subfigure}[b]{0.20 \textwidth}
                \includegraphics[scale=0.14]{illustration/HO-L.png}
                \caption{}
                \label{subfig:HO-L2}
            \end{subfigure}
            %
            \begin{subfigure}[b]{0.20 \textwidth}
                \includegraphics[scale=0.14]{illustration/HO-C.png}
                \caption{}
                \label{subfig:HO-C2}
            \end{subfigure}
            %
            \begin{subfigure}[b]{0.20 \textwidth}
                \includegraphics[scale=0.14]{illustration/HO-W.png}
                \caption{}
                \label{subfig:HO-W2}
            \end{subfigure}
            \caption{Caption}
            \label{fig:HO-all2}
        \end{figure}

\subsection{Isosurface Comparison}
%
Understanding and visualizing the linear interpolation error, the differences between the interpolation methods, and the effect of the feature recovery provide insights into the variability of the methods used for extracting the isosurfaces.
%
This information can be employed to guide decisions downstream in the pipeline.

[The framework name ] enables the comparison of isosurfaces obtained from different interpolation methods, as shown in [Figures].
\begin{itemize}
    \item AMR comparison
    \item HO comparison
\end{itemize}


\subsection{Isosurface Features Comparison}
%
Understanding the topological differences form using cell refinement, and different interpolation methods provides further insight into isosurface variability.
%
\begin{itemize}
    \item AMR comparison critical points
    \item HO comparison  critical points
\end{itemize}



==> old/todo.tex <==
\section{To Do}

\subsection{Error Approximation}
\begin{enumerate}
    \item clear argument for error approximation
    \item 
\end{enumerate}
\subsection{Interface}
\begin{enumerate}
    \item Statistics Summary
    \item Isosurface critical points visualization
    \item drop-down visualization update
    \item Adaptive refinement Visualization
\end{enumerate}

\subsection{Implementations}

\begin{enumerate}
    \item 3D adaptive refine for sharp feature recovery
    \item Isosurface critical points extractions
    \item Isosurface duplicate removal
    \item 
\end{enumerate}

\subsection{More Examples}
\subsubsection{Synthetic Examples}

\subsubsection{Real World Examples}
\begin{itemize}
    \item Engine dataset
\end{itemize}



\section*{Key Words}
\begin{enumerate}
    \item Adaptive Interpolation
    \item Adaptive Refinement/ Cell subdivision
    \item hidden extrema / hidden features
    \item Isosurface variability/ uncertainty
    \item Adaptive Interpolation for Marching Cubes
    \item Interactive Isosurface Analysis (Surface variability/Analysis)
    \item Linear Interpolation error
    \item Adaptive Interpolation
    \item Uncertainty guided HO interpolation for isosurface extraction
    \item Isosurface Uncertainty from Linear and  high order Interpolation
    \item Uncertainty Guided High Order Interpolation for Isosurface Extraction
    \item Estimation and Visualization of Isosurface Uncertainty From Linear and Higher Order Interpolation Model 
\end{enumerate}
%
